In Search of a Data Transformation That Accelerates Neural Field Training

Neural field is an emerging paradigm in data representation that trains a neural network to approximate the given signal. A key obstacle that prevents its widespread adoption is the encoding speed-generating neural fields requires an overfitting of a neural network, which can take a significant number of SGD steps to reach the desired fidelity level. In this paper, we delve into the impacts of data transformations on the speed of neural field training, specifically focusing on how permuting pixel locations affect the convergence speed of SGD. Counterintuitively, we find that randomly permuting the pixel locations can considerably accelerate the training. To explain this phenomenon, we examine the neural field training through the lens of PSNR curves, loss landscapes, and error patterns. Our analyses suggest that the random pixel permutations remove the easy-to-fit patterns, which facilitate easy optimization in the early stage but hinder capturing fine details of the signal.

==> assets/rebuttal/tables/denoising.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\renewcommand{\arraystretch}{1.2}
\begin{table}[h]
\centering
\resizebox{0.35\textwidth}{!}{%
\begin{tabular}{@{}lrrr}
\hline
            & Kodak & DIV2K & CLIC \\ \hline
{\rpp}  & 50dB  & 50dB & 50dB \\
Masked \citep{mask_denoise} & 28.71dB  & 28.02dB & 28.81dB \\
Self2Self \citep{self2self} & 28.25dB  & 27.58dB & 28.99dB \\
LG-BPN \citep{lgbpn} & 28.26dB  & 26.79dB & 28.21dB \\
 \hline 
\end{tabular}
}

\vspace{-0.5em}
\caption{PSNR after denoising, when applied on PSNR 30 images.}
%\caption{\textbf{Peak Signal-to-Noise Ratio (PSNR) of denoising algorithm.} We calculate the PSNR after applying a denoising algorithm to the reconstructed images which have 30dB of PSNR compared to target images. The symbol $\dagger$ denotes datasets that have been pretrained with the DND dataset.}
\label{table:denoising}
\vspace{-1em}
\end{table}

==> assets/rebuttal/tables/memory_usage.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\renewcommand{\arraystretch}{1.2}
\begin{table}[h]
\centering
\vspace{-1em}
\resizebox{0.49\textwidth}{!}{%
%\begin{tabular}{@{}lccc}
%\hline
%                   & FLOPs & Memory & Extra Rendering Compute \\ \hline
%SIREN        & 51.5T    & 790K    &   $207$G          \\ 
%Self2Self        & 49.27P    & 790K + 1375K    &   $207+107$G          \\ 
%LG-BPN  & pretrained   & 790K + 4560K    & $207+2670$G            \\ \hline
%\end{tabular}

\begin{tabular}{@{}lrr|rrr}
\hline
 & Dec. compute & Req. memory & Kodak & DIV2K & CLIC\\
\hline
{\rpp} & 207 GFLOPs & 790KB & 50 dB & 50dB & 50dB\\ 
Masked \citep{mask_denoise} & 631 GFLOPs & 1,614KB & 28.71dB & 28.02dB & 28.81dB\\
Self2Self \citep{self2self} & 314 GFLOPs & 2,165KB & 28.25dB & 27.58dB & 28.99dB\\ 
LG-BPN \citep{lgbpn} & 2,877 GFLOPs & 5,350KB & 28.26dB & 26.79dB & 28.21dB\\
\hline
\end{tabular}
}

\vspace{-0.5em}
\caption{(Left) Computational and memory footprint of RPP and various denoising algorithms. (Right) PSNR after denoising, when applied on images trained to achieve 30dB.}\label{table:compfoot}
\vspace{-1em}
\end{table}

% \caption{\textbf{Computational footprint.} {\color{blue}We measure required computation. FLOPs denotes the required computation for training a model to represent high fidelity (e.g. SIREN needs 51.5TFLOPs for 30db $\to$ 50dB). We follow the official implementation and details (training steps). And memory means the number of parameters and we also measure the decoding FLOPs for rendering an image. As we mentioned, the denoising algorithms requires much more computation and memory than SIREN. And significant computation for high fidelity (actually not achieved) is needed when we not use pretrained model.} }

==> assets/tables/all_raw.tex <==
\begin{table}[t]
\caption{\textbf{Average speedup on Instant-NGP.} We measure how each image transformation affects the number of SGD steps until convergence on Kodak images, and report the average speedup ratio against the original image. The speedups are colored in {\color{TdGreen}green}, and the slowdowns are colored in {\color{BrickRed}red.}}\label{tab:main}
  \centering
  \resizebox{0.45\textwidth}{!}{%
  \begin{tabular}{lccc}
    \toprule
    &Color Inversion & Random Perm. & Ordered Perm.\\
    \midrule
    Speedup &  {\color{BrickRed}0.123$\times$} & {\color{TdGreen}1.360$\times$} & {\color{BrickRed}0.765$\times$} \\
    \bottomrule
  \end{tabular}
  }
  \centering
\end{table}

==> assets/tables/bright_dark.tex <==
\begin{table}[t]
\caption{\textbf{Fitting darker/brighter images.} We measure how each image darkening or brightening transformations affect the training time. Note that, unlike prior tables and figures, we measure the number of SGD steps until achieving PSNR 50 on the \textit{transformed signal}, not on the original signal.}\label{tab:bd}
  \centering
  \resizebox{0.7\textwidth}{!}{%
  \begin{tabular}{cccccc}
    \toprule
    & \multirow{2}{*}{Halving} &
    \multicolumn{4}{c}{Gamma Correction}\\
    \cmidrule{3-6}
     & & \nicefrac{1}{4} & \nicefrac{1}{2} & \nicefrac{3}{2} & 2 \\
    \midrule
    Average Speedup &
    {\color{TdGreen}1.125$\times$} & {\color{TdGreen}2.178$\times$} & {\color{TdGreen}1.438$\times$} & {\color{BrickRed}0.766$\times$} & {\color{BrickRed}0.489$\times$}\\  \bottomrule
  \end{tabular}
  }
  \centering
\end{table}

==> assets/tables/correalations.tex <==
\begin{table}[]
\centering
\caption{Correlation of loss and the number of pixels.}
\begin{tabular}{@{}cccc@{}}
\toprule
        & Pearson & Spearman & P-value\\
\midrule
kodim01 & -0.338  & -0.334  & 2.06e-01\\
kodim02 & -0.197  & -0.968  & 9.13e-10\\
kodim03 & -0.355  & -0.556  & 2.54e-02\\
kodim04 & -0.265  & -0.947  & 2.72e-08\\
kodim05 & -0.341  & -0.956  & 7.76e-09\\
kodim06 & -0.308  & -0.576  & 1.94e-02 \\
kodim07 & -0.344  & -0.974  & 2.28e-10\\
kodim08 & -0.418  & -0.638  & 7.80e-03\\
kodim09 & -0.420  & -0.909  & 1.10e-06\\
kodim10 & -0.507  & -0.847  & 3.47e-05\\
kodim11 & -0.273  & -0.979  & 3.98e-11\\
kodim12 & -0.420  & -0.424  & 1.02e-01\\
kodim13 & -0.468  & -0.838  & 5.01e-05\\
kodim14 & -0.387  & -0.985  & 3.84e-12\\
kodim15 & -0.322  & -0.359  & 1.72e-01\\
kodim16 & -0.495  & -0.979  & 3.98e-11\\
kodim17 & -0.327  & -0.950  & 1.83e-08\\
kodim18 & -0.322  & -0.915  & 7.01e-07\\
kodim19 & -0.470  & -0.885  & 5.15e-06\\
kodim20 &  0.567  & -0.285  & 2.84e-01\\
kodim21 & -0.466  & -0.809  & 1.48e-04\\
kodim22 & -0.407  & -0.885  & 5.15e-06\\
kodim23 & -0.467  & -0.959  & 4.83e-09\\
kodim24 & -0.497  & -0.815  & 1.21e-04\\
\bottomrule
\end{tabular}
\end{table}


























==> assets/tables/cvpr/dct.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{table}[t]
\begin{tabular}{@{}lcc@{}}
\hline
      & \multicolumn{1}{c}{Original} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Random\\ Permutation\end{tabular}} \\ \hline
Kodak & 0.004                        & 0.119                                                                            \\ \hline
DIV2K & 0.012                        & 0.128                                                                            \\ \hline
CLIC  & 0.009                        & 0.129                                                                            \\ \hline                                                                     
\end{tabular}
\end{table}



==> assets/tables/cvpr/dct_1_low.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{table}[t]
\begin{tabular}{@{}lcc@{}}
\hline
            & \multicolumn{1}{c}{Original} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Random\\ Permutation\end{tabular}} \\ \hline
Kodak & 0.036                        & 0.357                                                                            \\ \hline
DIV2K & 0.059                        & 0.384                                                                            \\ \hline
CLIC  & 0.046                        & 0.386                                                                            \\ \hline                                                                 
\end{tabular}
\end{table}



==> assets/tables/cvpr/fixed_lr.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\renewcommand{\arraystretch}{1.2}
\begin{table*}[ht]

\centering
\resizebox{\textwidth}{!}{%

\begin{tabular}{@{}lcccccccccccc@{}}
\hline
                             \multirow{2}{*}{Architecture}& \multirow{2}{*}{Learning Rate}   & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Random\\ Permutation\end{tabular}} & \multirow{2}{*}{Zigzag} & \multirow{2}{*}{Inversion} & \multirow{2}{*}{Standardization} & \multicolumn{2}{c}{Linear Scaling} & \multicolumn{2}{c}{Centering} & \multicolumn{2}{c}{Gamma Correction} \\ \cline{7-12} 
                 &        &                                                                         &                         &                            &                                  & $t=0.5$             & $t=2.0$             & $t=1.0$               & $t=2.0$              & $\gamma=0.5$              & $\gamma=2.0$             \\ \hline

\multirow{3}{*}{SIREN} & $2^{-9}$   & N/A & N/A & N/A & N/A & N/A & N/A & N/A & N/A  & N/A  & N/A  \\
                       & $2^{-10}$       & \colorbox{blue!10}{1.29$_{3}$} & {3.72$_{1}$} & 0.82$_{2}$ & \colorbox{blue!10}{2.12$_{3}$} & 0.91$_{1}$ & \colorbox{blue!10}{1.43$_{2}$} & 0.78$_{2}$ & 0.88$_{4}$ & 0.92$_{21}$     & \colorbox{blue!10}{1.02$_{2}$} \\
                       & $2^{-11}$       &0.67$_{0}$ &  18.72$_{0}$ & 0.70$_{0}$ & \colorbox{blue!10}{3.18$_{0}$} & 0.67$_{0}$ & \colorbox{blue!10}{1.42$_{0}$} & 0.86$_{0}$ & \colorbox{blue!10}{1.27$_{0}$} & 0.58$_{1}$     & 0.92$_{0}$ \\
                       & $2^{-12}$       &0.55$_{21}$ &  56.79$_{0}$ & 0.91$_{2}$ & \colorbox{blue!10}{3.22$_{2}$} & 0.78$_{3}$ & \colorbox{blue!10}{1.55$_{2}$} & \colorbox{blue!10}{1.02$_{2}$} & \colorbox{blue!10}{1.25$_{2}$} & 0.69$_{6}$     & \colorbox{blue!10}{1.04$_{2}$} \\
\hline

\multirow{3}{*}{Instant-NGP} & $2^{-4}$  &\colorbox{blue!10}{2.16$_{1}$} & 0.58$_{2}$     & 0.22$_{19}$ & 0.30$_{5}$ & \colorbox{blue!10}{1.01$_{1}$} & \colorbox{blue!10}{1.07$_{2}$} & 0.55$_{10}$ & 0.51$_{8}$ & N/A$_{24}$ & 0.47$_{4}$ \\
                             & $2^{-5}$  &\colorbox{blue!10}{1.60$_{1}$} & 0.68$_{0}$     & 0.20$_{8}$ & 0.44$_{0}$ & 0.78$_{0}$ & 0.74$_{1}$ & \colorbox{blue!10}{1.12$_{0}$} & 0.52$_{0}$ & 0.20$_{21}$     & 0.39$_{1}$ \\
                             & $2^{-6}$  &\colorbox{blue!10}{1.67$_{0}$} & 0.89$_{0}$     & 0.17$_{13}$ & 0.44$_{0}$ & \colorbox{blue!10}{1.28$_{0}$} & 0.73$_{1}$ & \colorbox{blue!10}{1.27$_{0}$} & \colorbox{blue!10}{1.07$_{0}$} & 0.46$_{11}$     & 0.30$_{2}$ \\
\hline
\end{tabular}
}
\caption{\textbf{Average steps for achieving PSNR 50dB } The \colorbox{blue!10}{shaded} figures denote the speedup. }
\label{table:fixed_lr_siren_-9}
\end{table*}

==> assets/tables/main_results.tex <==
\begin{table}[t]
\caption{\textbf{Average Speedup Ratio.} We measure how each image transformation affects the number of SGD steps until convergence on Kodak images, and report the average speedup ratio against original. The speedups are colored in {\color{TdGreen}green}, and the slowdowns are colored in {\color{BrickRed}red.}}\label{tab:main}
  \centering
  \resizebox{0.98\textwidth}{!}{%
  \begin{tabular}{ccccccccc}
    \toprule
    \multirow{2}{*}{Halving} & \multirow{2}{*}{Centering} &
    \multicolumn{4}{c}{Gamma Correction}  & \multirow{2}{*}{Color Inv.} & \multirow{2}{*}{Random Perm.} & \multirow{2}{*}{Ordered Perm.} \\
    \cmidrule{3-6}
     & & \nicefrac{1}{4} & \nicefrac{1}{2} & \nicefrac{3}{2} & 2 & & & \\
    \midrule
    {\color{TdGreen}1.125$\times$} & {\color{BrickRed}0.771$\times$} & {\color{TdGreen}2.178$\times$} & {\color{TdGreen}1.438$\times$} & {\color{BrickRed}0.766$\times$} & {\color{BrickRed}0.489$\times$} &  {\color{BrickRed}0.123$\times$} & {\color{TdGreen}1.360$\times$} & {\color{BrickRed}0.765$\times$} \\
    \bottomrule
  \end{tabular}
  }
  \centering
\end{table}

==> assets/tables/reverse_all.tex <==
\begin{table}[h!]
\caption{Average Training steps for original \& reversed images}
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{cc}
    \toprule
    {Instant-NGP} & {SIREN}  \\
    \midrule
    VOID & 1.66 \\
    \bottomrule
  \end{tabular}
  }
  \centering
\end{table}

==> assets/tables/reverse_with40.tex <==
\begin{table}[h!]
\caption{Average Training steps for original \& reversed images}
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{ccc}
    \toprule
    {Target PSNR} & {Instant-NGP} & {SIREN}  \\
    \midrule
    PSNR40  & VOID & 1.43 \\
    \midrule
    PSNR50  & VOID & 1.93 \\
    \bottomrule
  \end{tabular}
  }
  \centering
\end{table}

==> assets/tables/shuffle_all.tex <==
\begin{table}[h!]
\caption{Average speedup in different architectures}
  \centering
  \begin{tabular}{cccc}
    \toprule
     \multirow{2}{*}{Instant-NGP} & \multirow{2}{*}{SIREN} & \multicolumn{2}{c}{FFN}  \\
    \cmidrule{3-4}
     &  & 10  & 15  \\
    \midrule
    1.36 $\times$ & 1.26 $\times$ & 0.82 $\times$ & 1.10 $\times$\\
    \bottomrule
  \end{tabular}
  \centering
\end{table}

==> assets/tables/shuffle_all2.tex <==
\begin{table}[t]
\centering
\caption{\textbf{Random permutation on various architectures.} We measure the average speedup from random permutation on various architectures, including the models that use sinusoidal encodings.}\label{tab:architectures}
\resizebox{0.47\textwidth}{!}{
\begin{tabular}{ccccc}
\toprule
 & Instant-NGP & SIREN & ReLU+P.E. ($m$=10) & ReLU+P.E. ($m$=15) \\
\midrule
Speedup & {\color{TdGreen}1.360$\times$} & {\color{TdGreen}1.265$\times$} & {\color{BrickRed}0.825$\times$} & {\color{TdGreen}1.099$\times$}\\
\bottomrule
\end{tabular}
}

\end{table}


==> assets/tables/shuffle_with40.tex <==
\begin{table}[h!]
\caption{Average Training steps for original \& shuffled images in different architectures}
  \centering
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{ccccc}
    \toprule
    \multirow{2}{*}{Target PSNR} & \multirow{2}{*}{Instant-NGP} & \multirow{2}{*}{SIREN} & \multicolumn{2}{c}{ReLU Network}  \\
    \cmidrule{4-5}
    &  &  & 10  & 15  \\
    \midrule
    PSNR40 & VOID & 3.13 & 1.46 & 0.99\\
    \midrule
    PSNR50 & VOID & 0.92 & 1.29 & 0.93\\
    \bottomrule
  \end{tabular}
  }
  \centering
\end{table}

==> assets/tables/siren_all_results.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{table}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llll@{}}

\toprule
\multicolumn{2}{l}{\textbf{Kodak dataset}}                                       & Average Steps & Average Speedup \\ \midrule
\multicolumn{2}{l}{Original}                                                     & 1371.375      & 1.000$\times$           \\ 
\multicolumn{2}{l}{\begin{tabular}[l]{@{}l@{}}Random Permutation\end{tabular}} & 1100.458      & {\color{TdGreen}1.265$\times}$           \\ 
\multicolumn{2}{l}{Zigzag}                                                       & 79.792        & {\color{TdGreen}17.902$\times}$          \\ 
\multicolumn{2}{l}{Inversion}                                                    & 2271.417      & {\color{BrickRed}0.720$\times}$           \\ 
\multicolumn{2}{l}{Standardization}                                              & 706.667       & {\color{TdGreen}2.204$\times}$           \\ 
\multicolumn{1}{l}{\multirow{2}{*}{Gamma Correction}}            & 0.5           & 4297.125      & {\color{BrickRed}0.355$\times}$           \\ 
\multicolumn{1}{l}{}                                             & 2.0           & 1835.375      & {\color{BrickRed}0.801$\times}$           \\ 
\multicolumn{1}{l}{\multirow{2}{*}{Linear Scaling}}              & 0.5           & 1875.208      & {\color{BrickRed}0.790$\times}$           \\  
\multicolumn{1}{l}{}                                             & 2.0           & 1051.042      & {\color{TdGreen}1.386$\times}$           \\ 
\multicolumn{1}{l}{\multirow{2}{*}{Centering}}                   & 1.0           &               &                 \\
\multicolumn{1}{l}{}                                             & 2.0           &               &                 \\ \bottomrule
\end{tabular}%
}
\end{table}
\renewcommand{\arraystretch}{1.0}

==> assets/tables/soaring.tex <==
\begin{table}[]
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lccc@{}}
\toprule
                  & \begin{tabular}[l]{@{}c@{}}Average Steps\\ for PSNR30\end{tabular} & \begin{tabular}[l]{@{}c@{}}Average Steps\\ for PSNR50\end{tabular} & Ratio \\ \midrule
Origin            & 105.8                                                            & 1371.4                                                           & 0.086 \\ 
Random Permutation & 851.8                                                            & 1100.5                                                           & 0.790 \\ \bottomrule
\end{tabular}%
}
\end{table}

==> assets/tables/total_result_steps_ngp.tex <==


\begin{table}[h!]
\caption{The number of steps to achieve target PSNR}
\label{appendix:total_step_ngp}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccccccc@{}}
\toprule
 & \multirow{2}{*}{Original} & \multicolumn{4}{c}{Gamma Correction} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Permutation\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}SIZZO\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Inversion\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Centering\end{tabular}} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Halving\end{tabular}} \\ 
 \cmidrule(l){3-6} &  & 0.25 & 0.5 & 1.5 & 2 &  &  &  &  &  \\ \midrule
Kodim01 & 69 & 15 & 43 & 126 & 264 & 68 & 83 & 15403 & 148 & 93 \\
Kodim02 & 118 & 62 & 66 & 73 & 149 & 80 & 140 & 13318 & 434 & 79 \\
Kodim03 & 112 & 45 & 60 & 175 & 211 & 81 & 150 & 12104 & 239 & 93 \\
Kodim04 & 134 & 70 & 94 & 144 & 200 & 81 & 208 & 15107 & 255 & 105 \\
Kodim05 & 119 & 69 & 82 & 105 & 230 & 95 & 160 & 4185 & 295 & 92 \\
Kodim06 & 347 & 107 & 219 & 473 & 504 & 190 & 305 & 1359 & 202 & 225 \\
Kodim07 & 107 & 80 & 90 & 131 & 255 & 71 & 87 & 2748 & 234 & 114 \\
Kodim08 & 202 & 94 & 149 & 301 & 414 & 205 & 294 & 1999 & 256 & 231 \\
Kodim09 & 131 & 81 & 127 & 373 & 601 & 126 & 288 & 1716 & 165 & 162 \\
Kodim10 & 177 & 74 & 126 & 336 & 582 & 120 & 256 & 4948 & 172 & 231 \\
Kodim11 & 146 & 72 & 114 & 124 & 210 & 90 & 145 & 2871 & 218 & 115 \\
Kodim12 & 392 & 101 & 240 & 631 & 1308 & 360 & 436 & 635 & 148 & 304 \\
Kodim13 & 194 & 73 & 96 & 249 & 338 & 111 & 286 & 930 & 256 & 197 \\
Kodim14 & 123 & 75 & 119 & 181 & 199 & 82 & 141 & 4571 & 189 & 118 \\
Kodim15 & 159 & 77 & 85 & 244 & 340 & 94 & 165 & 4835 & 535 & 105 \\
Kodim16 & 153 & 66 & 84 & 323 & 442 & 79 & 185 & 1951 & 234 & 138 \\
Kodim17 & 149 & 57 & 114 & 125 & 204 & 81 & 172 & 11163 & 231 & 110 \\
Kodim18 & 122 & 65 & 71 & 111 & 177 & 98 & 131 & 20997 & 339 & 78 \\
Kodim19 & 105 & 73 & 86 & 254 & 492 & 156 & 274 & 1095 & 178 & 204 \\
Kodim20 & 1234 & 1138 & 3940 & 1206 & 1555 & 4702 & 1686 & 1234 & 783 & 561 \\
Kodim21 & 121 & 77 & 116 & 224 & 360 & 79 & 254 & 1747 & 177 & 163 \\
Kodim22 & 106 & 71 & 110 & 215 & 426 & 93 & 257 & 1687 & 226 & 176 \\
Kodim23 & 214 & 84 & 108 & 261 & 452 & 123 & 286 & 1749 & 227 & 213 \\
Kodim24 & 142 & 84 & 89 & 317 & 385 & 140 & 255 & 12619 & 220 & 165 \\ 
\bottomrule
\end{tabular}
}
\centering
\end{table}


==> assets/tables/total_results_accelerate_ngp.tex <==
\begin{table}[h!]
\caption{Improvement ratios of transformed image compared to original}
\label{tab:total_accel_ngp}
\centering
\resizebox{\textwidth}{!}{%
    \begin{tabular}{@{}ccccccccccc@{}}
\toprule

\multirow{2}{*}{Image} & \multicolumn{4}{c}{Gamma Correction} & \multirow{2}{*}{\makecell{Permutation}} & \multirow{2}{*}{\makecell{SIZZO}} & \multirow{2}{*}{\makecell{Inversion}} & \multirow{2}{*}{\makecell{Centering}} & \multirow{2}{*}{\makecell{Halving}} \\ \cmidrule(lr){2-5}
 & 0.25 & 0.5 & 1.5 & 2 & & & & & \\ \midrule
Kodim01 & 4.600 $\times$ & 1.605 $\times$ & 0.548 $\times$ & 0.261 $\times$ & 1.015 $\times$ & 0.831 $\times$ & 0.004 $\times$ & 0.466 $\times$ & 0.742 $\times$ \\
Kodim02 & 1.903 $\times$ & 1.788 $\times$ & 1.616 $\times$ & 0.792 $\times$ & 1.475 $\times$ & 0.843 $\times$ & 0.009 $\times$ & 0.272 $\times$ & 1.494 $\times$ \\
Kodim03 & 2.489 $\times$ & 1.867 $\times$ & 0.640 $\times$ & 0.531 $\times$ & 1.383 $\times$ & 0.747 $\times$ & 0.009 $\times$ & 0.469 $\times$ & 1.204 $\times$ \\
Kodim04 & 1.914 $\times$ & 1.426 $\times$ & 0.931 $\times$ & 0.670 $\times$ & 1.654 $\times$ & 0.644 $\times$ & 0.009 $\times$ & 0.525 $\times$ & 1.276 $\times$ \\
Kodim05 & 1.725 $\times$ & 1.451 $\times$ & 1.133 $\times$ & 0.517 $\times$ & 1.253 $\times$ & 0.744 $\times$ & 0.028 $\times$ & 0.403 $\times$ & 1.293 $\times$ \\
Kodim06 & 3.243 $\times$ & 1.584 $\times$ & 0.734 $\times$ & 0.688 $\times$ & 1.826 $\times$ & 1.138 $\times$ & 0.255 $\times$ & 1.718 $\times$ & 1.542 $\times$ \\
Kodim07 & 1.338 $\times$ & 1.189 $\times$ & 0.817 $\times$ & 0.420 $\times$ & 1.507 $\times$ & 1.230 $\times$ & 0.039 $\times$ & 0.457 $\times$ & 0.939 $\times$ \\
Kodim08 & 2.149 $\times$ & 1.356 $\times$ & 0.671 $\times$ & 0.488 $\times$ & 0.985 $\times$ & 0.687 $\times$ & 0.101 $\times$ & 0.789 $\times$ & 0.874 $\times$ \\
Kodim09 & 1.617 $\times$ & 1.031 $\times$ & 0.351 $\times$ & 0.218 $\times$ & 1.040 $\times$ & 0.455 $\times$ & 0.076 $\times$ & 0.794 $\times$ & 0.809 $\times$ \\
Kodim10 & 2.392 $\times$ & 1.405 $\times$ & 0.527 $\times$ & 0.304 $\times$ & 1.475 $\times$ & 0.691 $\times$ & 0.036 $\times$ & 1.029 $\times$ & 0.766 $\times$ \\
Kodim11 & 2.028 $\times$ & 1.281 $\times$ & 1.177 $\times$ & 0.695 $\times$ & 1.622 $\times$ & 1.007 $\times$ & 0.051 $\times$ & 0.670 $\times$ & 1.270 $\times$ \\
Kodim12 & 3.881 $\times$ & 1.633 $\times$ & 0.621 $\times$ & 0.300 $\times$ & 1.089 $\times$ & 0.899 $\times$ & 0.617 $\times$ & 2.649 $\times$ & 1.289 $\times$ \\
Kodim13 & 2.658 $\times$ & 2.021 $\times$ & 0.779 $\times$ & 0.574 $\times$ & 1.748 $\times$ & 0.678 $\times$ & 0.209 $\times$ & 0.758 $\times$ & 0.985 $\times$ \\
Kodim14 & 1.640 $\times$ & 1.034 $\times$ & 0.680 $\times$ & 0.618 $\times$ & 1.500 $\times$ & 0.872 $\times$ & 0.027 $\times$ & 0.651 $\times$ & 1.042 $\times$ \\
Kodim15 & 2.065 $\times$ & 1.871 $\times$ & 0.652 $\times$ & 0.468 $\times$ & 1.691 $\times$ & 0.964 $\times$ & 0.033 $\times$ & 0.297 $\times$ & 1.514 $\times$ \\
Kodim16 & 2.318 $\times$ & 1.821 $\times$ & 0.474 $\times$ & 0.346 $\times$ & 1.937 $\times$ & 0.827 $\times$ & 0.078 $\times$ & 0.654 $\times$ & 1.109 $\times$ \\
Kodim17 & 2.614 $\times$ & 1.307 $\times$ & 1.192 $\times$ & 0.730 $\times$ & 1.840 $\times$ & 0.866 $\times$ & 0.013 $\times$ & 0.645 $\times$ & 1.355 $\times$ \\
Kodim18 & 1.877 $\times$ & 1.718 $\times$ & 1.099 $\times$ & 0.689 $\times$ & 1.245 $\times$ & 0.931 $\times$ & 0.006 $\times$ & 0.360 $\times$ & 1.564 $\times$ \\
Kodim19 & 1.438 $\times$ & 1.221 $\times$ & 0.413 $\times$ & 0.213 $\times$ & 0.673 $\times$ & 0.383 $\times$ & 0.096 $\times$ & 0.590 $\times$ & 0.515 $\times$ \\
Kodim20 & 1.084 $\times$ & 0.313 $\times$ & 1.023 $\times$ & 0.794 $\times$ & 0.262 $\times$ & 0.732 $\times$ & 1.000 $\times$ & 1.576 $\times$ & 2.200 $\times$ \\
Kodim21 & 1.571 $\times$ & 1.043 $\times$ & 0.540 $\times$ & 0.336 $\times$ & 1.532 $\times$ & 0.476 $\times$ & 0.069 $\times$ & 0.684 $\times$ & 0.742 $\times$ \\
Kodim22 & 1.493 $\times$ & 0.964 $\times$ & 0.493 $\times$ & 0.249 $\times$ & 1.140 $\times$ & 0.412 $\times$ & 0.063 $\times$ & 0.469 $\times$ & 0.602 $\times$ \\
Kodim23 & 2.548 $\times$ & 1.981 $\times$ & 0.820 $\times$ & 0.473 $\times$ & 1.740 $\times$ & 0.748 $\times$ & 0.122 $\times$ & 0.943 $\times$ & 1.005 $\times$ \\
Kodim24 & 1.690 $\times$ & 1.596 $\times$ & 0.448 $\times$ & 0.369 $\times$ & 1.014 $\times$ & 0.557 $\times$ & 0.011 $\times$ & 0.645 $\times$ & 0.861 $\times$ \\
\midrule
Average & 2.178 $\times$ & 1.438 $\times$ & 0.766 $\times$ & 0.489 $\times$ & 1.360 $\times$ & 0.765 $\times$ & 0.123 $\times$ & 0.771 $\times$ & 1.125 $\times$ \\
    \bottomrule
    \end{tabular}
}
\end{table}

==> assets/tables/total_results_percent_ngp.tex <==
\begin{table}[h!]
\caption{Computational cost ratios of transformed image compared to original}
\label{tab:total_percent_ngp}
\centering
\resizebox{\textwidth}{!}{%
    \begin{tabular}{@{}ccccccccccc@{}}
\toprule

\multirow{2}{*}{Image} & \multicolumn{4}{c}{Gamma Correction} & \multirow{2}{*}{\makecell{Permutation}} & \multirow{2}{*}{\makecell{SIZZO}} & \multirow{2}{*}{\makecell{Inversion}} & \multirow{2}{*}{\makecell{Centering}} & \multirow{2}{*}{\makecell{Halving}} \\ \cmidrule(lr){2-5}
 & 0.25 & 0.5 & 1.5 & 2 & & & & & \\ \midrule
Kodim01 & 0.217 & 0.623 & 1.826 & 3.826 & 0.986 & 1.203 & 223.232 & 2.145 & 1.348 \\
Kodim02 & 0.525 & 0.559 & 0.619 & 1.263 & 0.678 & 1.186 & 112.864 & 3.678 & 0.669 \\
Kodim03 & 0.402 & 0.536 & 1.563 & 1.884 & 0.723 & 1.339 & 108.071 & 2.134 & 0.830 \\
Kodim04 & 0.522 & 0.701 & 1.075 & 1.493 & 0.604 & 1.552 & 112.739 & 1.903 & 0.784 \\
Kodim05 & 0.580 & 0.689 & 0.882 & 1.933 & 0.798 & 1.345 & 35.168 & 2.479 & 0.773 \\
Kodim06 & 0.308 & 0.631 & 1.363 & 1.452 & 0.548 & 0.879 & 3.916 & 0.582 & 0.648 \\
Kodim07 & 0.748 & 0.841 & 1.224 & 2.383 & 0.664 & 0.813 & 25.682 & 2.187 & 1.065 \\
Kodim08 & 0.465 & 0.738 & 1.490 & 2.050 & 1.015 & 1.455 & 9.896 & 1.267 & 1.144 \\
Kodim09 & 0.618 & 0.969 & 2.847 & 4.588 & 0.962 & 2.198 & 13.099 & 1.260 & 1.237 \\
Kodim10 & 0.418 & 0.712 & 1.898 & 3.288 & 0.678 & 1.446 & 27.955 & 0.972 & 1.305 \\
Kodim11 & 0.493 & 0.781 & 0.849 & 1.438 & 0.616 & 0.993 & 19.664 & 1.493 & 0.788 \\
Kodim12 & 0.258 & 0.612 & 1.610 & 3.337 & 0.918 & 1.112 & 1.620 & 0.378 & 0.776 \\
Kodim13 & 0.376 & 0.495 & 1.284 & 1.742 & 0.572 & 1.474 & 4.794 & 1.320 & 1.015 \\
Kodim14 & 0.610 & 0.967 & 1.472 & 1.618 & 0.667 & 1.146 & 37.163 & 1.537 & 0.959 \\
Kodim15 & 0.484 & 0.535 & 1.535 & 2.138 & 0.591 & 1.038 & 30.409 & 3.365 & 0.660 \\
Kodim16 & 0.431 & 0.549 & 2.111 & 2.889 & 0.516 & 1.209 & 12.752 & 1.529 & 0.902 \\
Kodim17 & 0.383 & 0.765 & 0.839 & 1.369 & 0.544 & 1.154 & 74.919 & 1.550 & 0.738 \\
Kodim18 & 0.533 & 0.582 & 0.910 & 1.451 & 0.803 & 1.074 & 172.107 & 2.779 & 0.639 \\
Kodim19 & 0.695 & 0.819 & 2.419 & 4.686 & 1.486 & 2.610 & 10.429 & 1.695 & 1.943 \\
Kodim20 & 0.922 & 3.193 & 0.977 & 1.260 & 3.810 & 1.366 & 1.000 & 0.635 & 0.455 \\
Kodim21 & 0.636 & 0.959 & 1.851 & 2.975 & 0.653 & 2.099 & 14.438 & 1.463 & 1.347 \\
Kodim22 & 0.670 & 1.038 & 2.028 & 4.019 & 0.877 & 2.425 & 15.915 & 2.132 & 1.660 \\
Kodim23 & 0.393 & 0.505 & 1.220 & 2.112 & 0.575 & 1.336 & 8.173 & 1.061 & 0.995 \\
Kodim24 & 0.592 & 0.627 & 2.232 & 2.711 & 0.986 & 1.796 & 88.866 & 1.549 & 1.162 \\
\midrule
Average & 0.512 & 0.809 & 1.505 & 2.413 & 0.886 & 1.427 & 48.536 & 1.712 & 0.993 \\
    \bottomrule
    \end{tabular}
}
\end{table}

==> assets/tex/acceleration_ratio.tex <==
\begin{figure}[]
\centering
\includegraphics[width=0.4\linewidth]{assets/file/accelerate ratio_v3.pdf}
\caption{Speedup ratio over original image}
\label{fig:deprecated_acceleartion ratio}
\end{figure}


==> assets/tex/architecture_and_example.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{assets/file/pipeline_v1.pdf}
\caption{\textbf{Overall pipeline.} We consider fitting a neural field to a data transformed via some invertible mapping; the original data can be recovered by transforming back the data rendered by the neural field (left). By selecting the data transformation carefully, we can significantly reduce the number of SGD steps required to achieve a specific approximation quality (right).}
\label{fig:deprecated_pipeline}
\end{figure}

==> assets/tex/average_loss_for_mag.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.5\linewidth]{assets/file/Average Loss.pdf}
\caption{\textbf{Intensity vs. Loss.} We report the average squared losses of the pixels that have similar intensities. Lower index correspond to lower intensities.}
\label{fig:deprecated_average_loss}
\end{figure}

==> assets/tex/computational_cost_ratio.tex <==
\begin{figure}[H]
\centering
\includegraphics[width=0.7\linewidth]{assets/file/computational cost ratio.pdf}
\label{fig:deprecated_step ratio}
\end{figure}

==> assets/tex/cvpr_tex/kde_siren_kodak.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.95\linewidth]{assets/file/cvpr_figure/kde_siren_kodak.pdf}
\caption{{\color{ForestGreen}\textbf{Kernel Density Estimation} of Kodak dataset with SIREN architecture }}
\label{fig:kde_siren_kodak}
\end{figure}

==> assets/tex/permutation_results.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.98\linewidth]{assets/file/PERMUTATION_v2.pdf}
\caption{\textbf{Per-image speedup from random permutation (left).} We measure the average speedup provided by the random permutation. We observe more than $+50\%$ speedup on almost half of the images. \textbf{The effect of batch size on permutation-based speedup (right).} Randomly pixel-permuted images can be fit better with large batch sizes, while the images transformed via ordered permutation can be fit better with smaller batches.}
\label{fig:deprecated_acceleration ratio}
\end{figure}


==> sec/3_methodology.tex <==
\section{Methodology}

In this paper, as a preliminary step to solve the problem~\ref{eq:goal}, we focus on the \textit{proof-of-concept} that there exists some transformation such that the training cost reduces over the vanilla neural field training. More specifically, we show that there exists some choice of $T$ such that
\begin{align}
\mathsf{cost}(\mathbf{x},T) < \mathsf{cost}(\mathbf{x},\mathrm{Id}) \label{eq:whatwedo}
\end{align}
under a specific choice of the neural field architecture, signal and the cost function. More specifically, we focus on the task of 2D image regression, and measure the \textit{number of SGD steps} required to reach training PSNR 50, given the optimal learning rate (tuned from $\{2^{-4},\ldots,2^{-13}\}$); the number of SGD steps is an informative indicator of the total FLOPs and runtime for any fixed choice of hardware, model architecture, and data. Other experimental configurations are as follows.

\textbf{Data.} We use the Kodak image dataset \citep{kodak}, processed by center-cropping the $512\times512$ patch from each image and then converting to grayscale. The intensities of each pixel lie in the interval $[0,1]$.

\textbf{Model.} We mainly use a recently proposed neural field architecture based on the multi-resolution hash encoding, called Instant-NGP \citep{instantngp}. In some experiments, we additionally consider SIREN \citep{siren} and ReLU networks with sinusoidal positional encodings \citep{nerf}.

\textbf{Training.} We train the neural field using the mini-batch gradient descent. We use full-batch as a default (i.e., $2^{18}$), as this typically minimizes the number of required iterations. We also additionally consider the batch sizes $\{2^{12},2^{15}\}$ to gauge the impact of batch size on the acceleration from data transformations. To sample the data batch, we sample directly from coordinate points, instead of sampling from an interpolated version of the target image (used, e.g., in Instant-NGP \citep{instantngp}).

\input{assets/tables/all_raw}


\textbf{Data Transformations.}
%We consider total six transformations: Four transformations that change the intensity values (centering, halving, color inversion, gamma correction), and two transformations that only changes the location of the pixels (random permutation, ordered permutation).
We consider total three transformations. 
\begin{itemize}[leftmargin=*,topsep=0pt,parsep=0pt]
%\item \textit{Halving}: We reduce the intensities of each pixel to half, i.e., we apply $z \mapsto z/2$ to each pixel. The inverse transformation is to apply $z \mapsto 2z$ pixelwise.
%\item \textit{Centering}: We linearly scale-and-shift the intensities of the given image to the range $[-1,1]$. In other words, we apply $z \mapsto 2z-1$ pixelwise. The inverse transformation is to apply $z \mapsto (z+1)/2$.
\item \textbf{Color inversion}: We invert the target image, i.e., perform $z \mapsto 1-z$ on the pixel-wise intensity values. The inverse transformation is identical to the transformation itself.
%\item \textit{Gamma correction}: We nonlinearly scale the intensity of each pixels as $z \mapsto z^{1/\gamma}$, with the choice of $\gamma \in \{\nicefrac{1}{4},\nicefrac{1}{2},\nicefrac{3}{2},2\}$. Choosing $\gamma > 1$ makes images brighter, and $\gamma < 1$ makes darker. The inverse transformation is to apply $z \mapsto z^{\gamma}$ for each pixel.
\item \textbf{Random permutation}: We randomly permute the position of the pixels, while leaving the intensity values unchanged. The inverse transformation is to apply the transpose of the permutation matrix used for the original transformation. This transformation gives a high-frequency image.
\item \textbf{Ordered permutation}: We first sort the pixels by their intensities in an ascending order, and place the first pixel at the top-left corner, i.e., a $1\times1$ square. Then, we consider a larger $2\times 2$ square on top-left, and fill the remaining $\sansLmirrored$-shaped region with the next three pixels in the clockwise order (i.e., $\carriagereturn$). Then, we fill the remaining $\sansLmirrored$-shaped pixels of $3\times 3$ square, but in a counterclockwise order. We repeat this process until the full image is filled. This gives a low-frequency image.
\end{itemize}



%\textbf{Hyperparameters.} We train the model using the learning rates in the range $\{2^{-4},\ldots,2^{-13}\}$, and report the best performance (i.e., smallest number of steps until PSNR 50).

%To investigate which data transformation accelerates neural field training, we conduct experiments on the 512 $\times$ 512 center-cropped Kodak images. \citep{kodak} For a more in-depth analysis of loss values in relation to intensity levels, these images were converted into grayscale.

%Our work focuses on fitting an image of neural fields, and experiments are conducted employing the framework of Instant-NGP\citep{instantngp}, which uses multi-resolution hash encoding. Instant-NGP fits an image by randomly sampling coordinates with replacement, but in our experiments, we fit the image with fixed coordinates without replacement, which is mostly used in neural network training. Also, since the sampled coordinates are not located at the center of the grid, bilinear interpolation is used in Instant-NGP, but we perform the experiments without interpolation.


%To represent an image with neural field, we need to train the network for each image, so we found the optimal learning rate in [2$^{-4}$ -- 2$^{-13}$] for a fair comparison. Also, to scrutinize the impact of batch size, we conducted experiments with batch sizes of [2$^{12}$, 2$^{15}$, 2$^{18}$].



%We measured the number of steps required to satisfy the target psnr because the image represented by the neural field should satisfy a certain quality level, and investigated which data transformation accelerates neural field training.



%\textbf{Gamma correction} serves as a technique to modulate image brightness, with the study exploring Gamma values of [0.25, 0.5, 1.5, 2.0]. \textbf{Random permutation} was used to randomly change the position of the pixel while leaving the color unchanged. The permutation transformation was used to investigate how the neural field behaves when an image loses semantic information and thus lacks continuity in local color similarity. \textbf{Inversion} was deployed to reverse the color scheme within images. A strategy named \textbf{Zigzag low-frequency} sorted the pixels in the image in order of intensity and permuted the image pixels in a zigzag order. This systematic method allowed us to characterize the image as sharing identical pixel colors with low-frequency features.

==> sec/4_findings.tex <==
%\input{assets/tables/main_results}



\section{Observations}
\label{Findings}

We summarize the empirical findings in \Cref{tab:main}. We observe that, in general, applying data transformations has a huge impact on the number of SGD steps until achieving certain PSNR levels, from slowing down the training by $\sim88\%$, to speeding up the training by $36\%$.

We especially find two observations noteworthy, and take a closer look at each with the follow-up experiments. For each observation, we provide a preliminary hypothesis to explain the phenomenon.

\subsection{Randomly pixel-permuted images can be fit faster}

\input{assets/tex/permutation_results}

To our surprise, random pixel permutations often makes the image training much faster than the original image. In the left of \Cref{fig:acceleration ratio}, we report the per-image acceleration ratio due to pixel permutation. On 21 out of 24 images, we observe a speedup, sometimes as significant as $+93.7\%$ (image\#16). In some images, however, there is an extreme slowdown; $-32.7\%$ on image\#19, and $-73.8\%$ on image\#20. In contrast, ordered permutation slows down the training with $-23.5\%$.

From the \textit{frequency perspective}, this is a very intriguing phenomenon; are higher-frequency images easier to fit? Random pixel-permutation give high-frequency images---if we measure the signal intensity of the high-frequency component via discrete cosine transform (DCT),\footnote{We measure this as follows: we divide each image into $8\times8$ patches and compute the DCT coefficients. We compute the sum of squared coefficients, except for the low-frequency region (i.e., the upper-left quarter).} randomly permuted images gives the intensity 35.67, which is very large compared with the 3.58 of the original images. The ordered permutation gives a much lower-frequency, with the high-frequency intensity 0.03. In this sense, our observation is contrary to the common belief that low-frequency images fit faster.

\input{assets/tables/shuffle_all2}

To better understand when and why such counterintuitive phenomenon happens, we have conducted follow-up experiments to identify two components that affect the efficacy of random permutation.
\begin{itemize}[leftmargin=*,parsep=0pt,topsep=0pt]
\item \textbf{Batch size:} We observe that the tendency to fit randomly pixel-permuted images better is largely a batch-size-dependent phenomenon (right of \Cref{fig:acceleration ratio}). For larger batch sizes, randomly pixel-permuted images are trained faster. For smaller batch sizes, orderedly pixel-permuted images tend to fit much faster, $11\times$ faster on average. In contrast, random permutation slows down the training. We hypothesize that small batch size introduces large SGD noise, which prevents the model from fitting the high-frequency signals.
\item \textbf{Architecture.} We also find that the speedup from random permutations is largely a architecture-dependent issue (\Cref{tab:architectures}). The models which have a better expressive capacity tend to work better with randomly pixel-permuted images; this is most evident in the case of ReLU networks with positional encodings \citep{nerf}, where we test with two different choices of the number of sinusoidal bases ($m = 10, 15$). The model with larger number of bases can be accelerated by random pixels, but the model with a smaller number of bases is slowed down.
\end{itemize}
From these observations, we hypothesize that random permutations accelerate training by helping the model better utilize its capacity to express high-frequency components, which is typically underutilized in many cases. With small batch sizes, the SGD noise becomes too large so that it reduces the capacity of the models to fit high-frequency signals; the ability to fit low-frequency signals (for some reason) tends to be more robust to such noise.

\subsection{Inverted images fit much slower}
We also find that the inverted images fit much slower than the original images; original images require only around $12.3\%$ of the SGD steps required to fit the inverted images. The only exception is Kodak image\#20, where the number of required SGD steps remains almost identical. This observation has almost nothing to do with the frequency, as the inverted image has mostly identical frequency patterns, except for the zero-frequency component.

We hypothesize that this is due to the \textit{magnitude bias}: the pixels with larger intensity are more difficult to fit. To back-up this point, we conduct two follow-up analyses.

\input{assets/tables/bright_dark}
\input{assets/tex/average_loss_for_mag}

\begin{itemize}[leftmargin=*,topsep=0pt,parsep=0pt]
\item \textbf{Darkening / Brightening transformations.} We compare the number of SGD steps required to fit the ``darkened'' or ``brightened'' of each image. As such transformations, we consider either halving the intensity values (i.e., $z \mapsto \nicefrac{z}{2}$), or applying gamma correction (i.e., $z \mapsto z^{1/\gamma}$). The results are given in \Cref{tab:bd}. We confirm that the images with darker pixels are easier to fit, and images with brighter pixels are much more difficult to fit.
\item \textbf{Intensity-to-loss relationship.} We quantize the intensity range $[0,1]$ into $16$ uniform intervals, and report the average loss of the pixels whose intensity belong to the each interval (when trained on original images). We report the results in \Cref{fig:average_loss}. From the figure, we observe that the average losses are much higher in the pixels that have higher intensity values, concluding that neural fields find it more difficult to fit larger-magnitude functions.
\end{itemize}




%Table 2 demonstrates the influence of changing intensity distributions on the speed of training. Remarkably, reducing the value of the gamma correction speeds up the learning process.  In contrast, higher gamma values, which yield brighter images, slow down the model fitting significantly. And the inversion transformation tends to fit slowly.  An examination of intensity values within the Kodak image shows that the distribution is concentrated at lower intensities. However, under the inversion transformation, there is a distinct shift: the intensity distribution inverts, concentrating predominantly at higher values. This inversion of intensities mirrors the results of the gamma correction experiments, which indicates a challenge in fitting high intensity images. Furthermore, a transformation dubbed 'halving', which reduce the intensity by half, also yields an acceleration. This observation aligns coherently with the results of gamma correction.

% Show the Quantization graph and the experiments for reversed images. The number of steps to converge increases as the image becomes brighter(reversed). We'll explain that high intensity is harder to fit when the number of pixels is similar.
% Additionally, I'm considering whether to include this. How "srgb to linear rgb" could actually help train.


%\subsubsection{in-depth analysis of loss map}
%Figure~\ref{fig:average_loss} shows that the relationship between pixel intensity and loss. To calculate, the intensity range $[-1,1]$ is segmented into 16 discrete intervals, and the average loss is computed for pixels residing within each respective interval. Subsequent to this calculation, normalization is conducted within each intensity grid to facilitate comparability across diverse intensity values. Finally, an aggregate mean is derived for each grid by averaging the normalized values across all images, thereby providing a consolidated view of intensity-dependent loss dynamics within the Kodak images. This observation highlights a direct correlation between pixel intensity and loss magnitude, substantiating the aforementioned results where images of lower intensity facilitate a more fast fitting process.

%\subsection{Pixel Imbalance: Minority colors are fit slower than majority colors}
%We investigated the relation between pixel quantity within each intensity grid and the corresponding grid's average loss value. Within machine learning paradigms, minority classes frequently encounter diminished predictive accuracy. \citep{groupdro} This issue can be attributed, in part, to discrepancies in the distribution between training and testing dataset. Intriguingly, we found a similar dynamic in our experiments where there was no dicrepancy. In pursuit of quantitatively substantiating this observed phenomenon, we calculated both Pearson and Spearman correlation coefficients for each image under consideration. The computed average Pearson and Spearman correlation coefficients across the images were -0.343 and -0.782 respectively, providing numerical evidence supporting the hypothesis of slower fitting speeds for minority colors due to the observed pixel imbalance. 



